Disentangling the Galaxy's Gordian knot: evidence from $APOGEE-Gaia$ for a knotted and slower bar in the Milky Way

The inner $\sim5$ kiloparsec (kpc) region of the Milky Way is complex. Unravelling the evolution of the Galaxy requires precise understanding of the formation of this region. We report a study focused on disentangling the inner Galaxy ($r < 5$ kpc) using the measured positions, velocities, and element abundance ratios of red giant stars from the $APOGEE-Gaia$ surveys. After removing the stellar halo, inner Galaxy populations can be grouped into three main components based on their angular momentum: bar, disc, and a previously unreported ``knot'' component. The knot has a spheroidal shape, is concentrated in the inner $\sim1.5$ kpc, is comprised of stars on nearly-radial orbits, and contains stars with super-solar [Fe/H] element abundances. The chemical compositions of the knot are qualitatively similar to the Galactic bar and inner disc, suggestive that these three populations share a common genesis; the chemical/dynamic properties of the knot suggest it could constitute a classical bulge formed via secular evolution. Moreover, our results show that the bar is more slowly rotating than previously thought, with a pattern speed of $\Omega_{\mathrm{bar}}=24\pm3$ km s$^{-1}$ kpc$^{-1}$. This new estimate suggests that the influence of the bar extends beyond the solar radius, with $R_{\mathrm{CR}}\sim9.4-9.8$ kpc, depending on the adopted Milky Way rotation curve; it also suggests a ratio of corotation to bar length of $\mathcal{R}\sim1.8-2$. Our findings help place constraints on the formation and evolution of inner Galaxy populations, and directly constrain dynamical studies of the Milky Way bar and stars in the solar neighbourhood.

==> tables/fittable.tex <==
\begin{table*}
\centering
  \begin{tabular}{l|l|l|l|l|l|l|l|l|l}
  \hline
 name & radii& $f$ & L$_x$ & L$_y$ & L$_z$ & $\gamma$ & $\sigma_x$ & $\sigma_y$ & $\sigma_z$ \\
 &[kpc] & [$\%$] & [$\kpc~\kms$]& [$\kpc~\kms$] & [$\kpc~\kms$] & [$^\circ$] & [$\kpc~\kms$] & [$\kpc~\kms$] &  [$\kpc~\kms$] \\
\hline
disc&$0.0-1.0$&$0.1596^{+0.0262}_{-0.0258}$&$1.8^{+12.4}_{-12.7}$&$9.3^{+12.0}_{-12.3}$&$92.8^{+10.1}_{-9.5}$&$24.2^{+16.5}_{-54.0}$&$130.4^{+14.1}_{-10.4}$&$142.3^{+13.7}_{-14.4}$&$41.7^{+6.3}_{-6.2}$\\
bar&$0.0-1.0$&$0.6136^{+0.0286}_{-0.0274}$&$2.5^{+3.2}_{-3.1}$&$2.2^{+2.4}_{-2.5}$&$11.7^{+2.8}_{-2.8}$&$38.8^{+3.6}_{-3.6}$&$80.3^{+3.0}_{-2.8}$&$55.7^{+3.0}_{-2.8}$&$30.8^{+2.5}_{-2.2}$\\
knot&$0.0-1.0$&$0.2274^{+0.0207}_{-0.0203}$&$-0.7^{+2.3}_{-1.0}$&$-0.8^{+1.5}_{-0.9}$&$0.0^{+0.8}_{-0.8}$&$33.5^{+5.1}_{-4.3}$&$25.8^{+2.8}_{-2.6}$&$10.5^{+0.9}_{-0.4}$&$10.1^{+0.2}_{-0.1}$\\
    \hline
disc&$0.5-1.5$&$0.1872^{+0.0207}_{-0.0212}$&$-3.7^{+10.0}_{-10.1}$&$9.3^{+10.7}_{-10.4}$&$117.1^{+7.9}_{-7.7}$&$31.6^{+12.4}_{-13.3}$&$150.3^{+8.4}_{-7.3}$&$173.8^{+10.4}_{-9.2}$&$69.4^{+6.3}_{-6.0}$\\
bar&$0.5-1.5$&$0.6185^{+0.0224}_{-0.0213}$&$2.5^{+3.0}_{-2.9}$&$2.8^{+2.4}_{-2.4}$&$25.5^{+2.9}_{-2.8}$&$35.4^{+3.6}_{-3.7}$&$83.2^{+2.7}_{-2.6}$&$59.9^{+2.6}_{-2.5}$&$42.0^{+2.2}_{-2.1}$\\
knot&$0.5-1.5$&$0.1941^{+0.0152}_{-0.0156}$&$-0.7^{+1.9}_{-1.5}$&$-3.0^{+1.4}_{-1.4}$&$0.3^{+0.9}_{-0.9}$&$31.8^{+4.6}_{-4.2}$&$25.2^{+2.3}_{-2.2}$&$10.6^{+1.0}_{-0.5}$&$10.1^{+0.2}_{-0.1}$\\
    \hline
disc&$1.0-2.0$&$0.3802^{+0.023}_{-0.0225}$&$-7.9^{+6.6}_{-6.4}$&$-1.2^{+7.7}_{-7.5}$&$160.8^{+6.4}_{-6.3}$&$44.7^{+29.0}_{-29.4}$&$154.2^{+5.3}_{-5.2}$&$158.6^{+5.7}_{-5.3}$&$89.5^{+4.4}_{-4.2}$\\
bar&$1.0-2.0$&$0.5005^{+0.0222}_{-0.0221}$&$2.9^{+3.2}_{-3.4}$&$-4.0^{+2.5}_{-2.6}$&$-0.6^{+3.5}_{-3.1}$&$40.1^{+3.9}_{-4.0}$&$80.5^{+2.9}_{-2.7}$&$56.3^{+2.9}_{-2.8}$&$44.2^{+2.6}_{-2.5}$\\
knot&$1.0-2.0$&$0.1198^{+0.0126}_{-0.0119}$&$0.1^{+0.8}_{-1.2}$&$-0.4^{+1.5}_{-0.6}$&$0.0^{+0.7}_{-0.8}$&$16.5^{+9.2}_{-9.4}$&$18.5^{+2.4}_{-2.0}$&$10.6^{+0.9}_{-0.5}$&$10.3^{+0.5}_{-0.2}$\\
    \hline
disc&$1.5-2.5$&$0.5688^{+0.0367}_{-0.0312}$&$-7.6^{+5.6}_{-5.6}$&$-4.3^{+5.3}_{-5.2}$&$210.8^{+7.0}_{-6.1}$&$52.8^{+12.9}_{-12.2}$&$168.0^{+4.7}_{-4.4}$&$155.4^{+4.9}_{-4.3}$&$128.4^{+4.6}_{-4.2}$\\
bar&$1.5-2.5$&$0.3506^{+0.0293}_{-0.0325}$&$4.0^{+4.6}_{-4.7}$&$-6.2^{+3.4}_{-3.4}$&$-9.6^{+8.0}_{-6.9}$&$58.5^{+4.3}_{-4.1}$&$89.3^{+5.0}_{-4.8}$&$58.0^{+4.9}_{-4.5}$&$59.9^{+5.5}_{-5.2}$\\
knot&$1.5-2.5$&$0.0818^{+0.01}_{-0.0095}$&$0.3^{+0.8}_{-1.8}$&$0.4^{+0.7}_{-1.5}$&$0.0^{+1.0}_{-1.1}$&$31.0^{+8.7}_{-7.8}$&$20.7^{+2.9}_{-2.7}$&$10.4^{+0.8}_{-0.3}$&$10.9^{+1.4}_{-0.7}$\\
    \hline
disc&$2.0-3.0$&$0.4845^{+0.034}_{-0.0366}$&$-10.6^{+6.6}_{-6.6}$&$-3.1^{+7.4}_{-6.5}$&$369.5^{+10.3}_{-10.4}$&$67.1^{+32.7}_{-14.2}$&$187.6^{+5.3}_{-5.4}$&$178.5^{+6.3}_{-5.6}$&$140.6^{+7.4}_{-6.5}$\\
bar&$2.0-3.0$&$0.4708^{+0.0357}_{-0.0332}$&$6.2^{+5.5}_{-5.3}$&$-1.6^{+3.5}_{-3.6}$&$156.7^{+8.7}_{-9.6}$&$75.8^{+2.4}_{-2.5}$&$140.3^{+4.8}_{-4.9}$&$88.0^{+3.8}_{-4.1}$&$136.8^{+4.6}_{-5.1}$\\
knot&$2.0-3.0$&$0.0443^{+0.0066}_{-0.0074}$&$2.0^{+3.5}_{-4.0}$&$-3.6^{+2.1}_{-2.1}$&$6.6^{+3.9}_{-3.7}$&$58.7^{+8.2}_{-7.0}$&$28.0^{+7.3}_{-6.1}$&$11.2^{+1.9}_{-0.9}$&$19.6^{+4.7}_{-3.7}$\\
    \hline
-&$2.5-3.5$&$0.0113^{+0.002}_{-0.0024}$&$-16.8^{+73.8}_{-61.6}$&$-365.2^{+35.2}_{-46.7}$&$-316.4^{+34.9}_{-36.8}$&$21.2^{+11.7}_{-13.2}$&$238.0^{+37.7}_{-28.6}$&$387.6^{+57.0}_{-53.6}$&$142.4^{+28.1}_{-22.4}$\\
disc&$2.5-3.5$&$0.6113^{+0.0325}_{-0.035}$&$-14.3^{+5.0}_{-5.0}$&$-4.3^{+3.7}_{-2.9}$&$476.9^{+9.1}_{-8.9}$&$78.6^{+5.5}_{-4.9}$&$195.8^{+3.6}_{-3.9}$&$171.9^{+4.2}_{-3.7}$&$158.0^{+4.7}_{-4.6}$\\
bar&$2.5-3.5$&$0.3774^{+0.0351}_{-0.0326}$&$2.0^{+5.8}_{-5.5}$&$0.3^{+3.3}_{-3.0}$&$215.3^{+11.8}_{-12.2}$&$80.7^{+1.6}_{-1.6}$&$157.9^{+4.7}_{-4.8}$&$77.5^{+3.8}_{-4.3}$&$148.6^{+6.1}_{-5.8}$\\
    \hline
disc&$3.0-4.0$&$0.6373^{+0.0302}_{-0.0305}$&$-20.4^{+4.3}_{-4.5}$&$-2.0^{+2.4}_{-1.4}$&$616.3^{+8.1}_{-8.3}$&$84.7^{+4.6}_{-3.6}$&$197.4^{+3.2}_{-3.1}$&$177.2^{+3.6}_{-3.2}$&$168.2^{+4.2}_{-3.9}$\\
-&$3.0-4.0$&$0.0157^{+0.0022}_{-0.0024}$&$32.7^{+36.9}_{-35.6}$&$-197.3^{+36.0}_{-39.8}$&$-257.5^{+27.8}_{-25.4}$&$22.9^{+7.5}_{-7.3}$&$206.7^{+22.6}_{-20.5}$&$355.5^{+36.3}_{-33.9}$&$165.9^{+22.7}_{-20.1}$\\
bar&$3.0-4.0$&$0.347^{+0.0313}_{-0.0303}$&$-9.1^{+6.1}_{-6.0}$&$-2.3^{+3.3}_{-3.2}$&$318.3^{+13.4}_{-14.0}$&$78.9^{+1.3}_{-1.3}$&$186.7^{+5.1}_{-4.8}$&$87.7^{+3.6}_{-3.9}$&$174.3^{+6.9}_{-6.4}$\\
    \hline
-&$3.5-4.5$&$0.0003^{+0.0002}_{-0.0002}$&$94.9^{+286.7}_{-260.9}$&$-528.0^{+54.6}_{-91.1}$&$-924.7^{+74.0}_{-75.3}$&$43.1^{+29.3}_{-29.4}$&$13.7^{+8.4}_{-2.8}$&$14.0^{+9.1}_{-3.1}$&$14.1^{+9.7}_{-3.1}$\\
-&$3.5-4.5$&$0.0003^{+0.0002}_{-0.0002}$&$-315.3^{+246.7}_{-350.6}$&$549.0^{+241.1}_{-94.8}$&$-375.8^{+38.5}_{-39.1}$&$44.1^{+28.7}_{-30.8}$&$14.5^{+10.3}_{-3.5}$&$14.3^{+9.3}_{-3.3}$&$14.2^{+9.3}_{-3.2}$\\
disc&$3.5-4.5$&$0.9994^{+0.0003}_{-0.0002}$&$-16.7^{+2.6}_{-2.8}$&$5.3^{+2.0}_{-2.1}$&$638.5^{+3.6}_{-3.6}$&$82.6^{+1.6}_{-1.6}$&$204.2^{+1.7}_{-1.9}$&$160.9^{+1.6}_{-1.6}$&$258.7^{+2.5}_{-2.4}$\\
    \hline
-&$4.0-5.0$&$0.0002^{+0.0001}_{-0.0002}$&$-443.2^{+380.9}_{-803.6}$&$-612.7^{+298.2}_{-380.7}$&$-406.0^{+373.3}_{-365.4}$&$35.8^{+14.5}_{-17.1}$&$10.4^{+0.3}_{-0.3}$&$10.5^{+0.6}_{-0.3}$&$11.4^{+0.4}_{-0.4}$\\
-&$4.0-5.0$&$0.0004^{+0.0002}_{-0.0003}$&$355.9^{+121.5}_{-102.1}$&$638.2^{+84.6}_{-108.2}$&$-395.1^{+258.5}_{-27.2}$&$9.4^{+5.8}_{-8.6}$&$17.3^{+8.5}_{-3.7}$&$11.0^{+1.1}_{-0.7}$&$24.2^{+14.9}_{-6.7}$\\
disc&$4.0-5.0$&$0.9994^{+0.0004}_{-0.0002}$&$-7.6^{+1.5}_{-1.6}$&$10.9^{+0.8}_{-0.8}$&$792.7^{+2.8}_{-2.8}$&$83.9^{+0.8}_{-0.6}$&$205.6^{+1.3}_{-1.2}$&$152.4^{+0.6}_{-0.6}$&$280.8^{+1.0}_{-0.9}$\\
  \hline
  \hline

\end{tabular}
  \caption{Values for parameters of interest derived from the GMM fits.}
  \label{tab:fitparams}
\end{table*}
